Rare events, time crystals and symmetry-breaking dynamical phase transitions

In this PhD thesis, I investigate the properties of symmetry-breaking dynamical phase transitions that manifest in the fluctuations of time-integrated observables within classical systems. In particular, I analyze how these phase transitions impose stringent constraints on the structure of the eigenvectors of the system dynamical generator of the dynamics. Additionally, I identify a dynamical phase transition to a time-crystal phase in a model of driven-diffusive lattice gas. The study of this transition then allows the identification of the "packing-field" mechanism responsible for its emergence. This mechanism is then exploited to propose new transport models displaying time-crystal behavior.

==> commands_WASEP.tex <==
% Travelling wave properties
\newcommand{\freqTW}{\alpha} % Frequency of the travelling wave (imaginary part of eigenvalue)
\newcommand{\velTW}{v_{\mathrm{TW}}} % Speed of the travelling wave

% Center of mass
\newcommand{\xCM}{X_{\mathrm{CM}}}
\newcommand{\xCMop}{\hat{X}_{\mathrm{CM}}}
\newcommand{\yCM}{Y_{\mathrm{CM}}}
\newcommand{\yCMop}{\hat{Y}_{\mathrm{CM}}}
\newcommand{\rCM}{r_{\mathrm{CM}}}
\newcommand{\rCMop}{\hat{r}_{\mathrm{CM}}}
\newcommand{\thetaCM}{\theta_{\mathrm{CM}}}
\newcommand{\thetaCMop}{\hat{\theta}_{\mathrm{CM}}}

% Equivalence class
\newcommand{\eqclasstrans}[1]{[#1]}

% Traslation operator
\newcommand{\translation}{T}
\newcommand{\translationop}{\hat{\translation}}
\newcommand{\transeigvalsymb}{t}
\newcommand{\transeigval}[1]{\transeigvalsymb_{#1}}
\newcommand{\transeigvalarg}[1]{\varphi^{\transeigvalsymb}_{#1}}


==> titlepage/titlepage.tex <==
\pagestyle{empty}
\makeatletter
    \centering

    \includegraphics[width=0.4\textwidth]{logo_ugr}
    \vspace{1cm}

	{\huge \textbf{\@title} \par} 

	\vspace{1cm}

	{\itshape \normalsize \setlength{\parskip}{0.2cm}
	    {\normalfont\large \textbf{DOCTORAL DISSERTATION}}

        presented to obtain the

        {\normalfont DOCTOR OF PHILOSOPHY DEGREE}

        in the 

	    {\normalfont \large Doctoral Programme in Physics and Mathematics (FisyMat)}

        by

	    {\normalfont \Large \bfseries \@author}

        %\vspace{1.\parskip}

        supervised by


	    {\normalfont \large 
            Pablo Ignacio Hurtado Fernández

            Carlos Pérez Espigares
        }
    }

    \vfill

    Granada, 2024
\makeatother

